Object-Centric Multi-Task Learning for Human Instances

Human is one of the most essential classes in visual recognition tasks such as detection, segmentation, and pose estimation. Although much effort has been put into individual tasks, multi-task learning for these three tasks has been rarely studied. In this paper, we explore a compact multi-task network architecture that maximally shares the parameters of the multiple tasks via object-centric learning. To this end, we propose a novel query design to encode the human instance information effectively, called human-centric query (HCQ). HCQ enables for the query to learn explicit and structural information of human as well such as keypoints. Besides, we utilize HCQ in prediction heads of the target tasks directly and also interweave HCQ with the deformable attention in Transformer decoders to exploit a well-learned object-centric representation. Experimental results show that the proposed multi-task network achieves comparable accuracy to state-of-the-art task-specific models in human detection, segmentation, and pose estimation task, while it consumes less computational costs.

==> intro_backup.tex <==
\section{Introduction}
\label{sec:intro}

% \jung{storyline 이 필요해 보임.
% - 예) DAB-DETR 의 경우 
% 1) DETR vs. Anchor-based Detection 소개, 2) 기존 DETR 의 단점, 3) 제안한 방법 간략 소개, 4) 그 의미, 5) 기존 단점 해결했어요, 6) Summary
% - 우리의 경우 (MTL) 관점의 예 
% 1) 기존 MTL 의 접근 방식 (큰 분류), 2) 기존 MTL 의 단점, 3) 제안한 MTL 간략 소개, 4) 제안한 방식의 동작 원리, 5) 어떻게 기존 MTL 단점을 해결했는가, 6) Summary 
% - Human Pose + Seg 관점의 예
% 1) 왜 Human Pose + Seg 인가, 2) 기존 P+S 접근 방식 분류, 3) 기존 방식 문제점, 4) 우리 방식 간략 소개, 5) 기존 단점을 어떻게  해결했는가?, 6) Summary 
% - Related Work 은 이 위 관점을 기준으로 분류하여 정리해야 할 듯 함

% Object-Centric Learning 
% 1) object-centric learning의 정의 및 MTL architecture로의 활용 가능성
%   : 정의 - query 가 object instance 대응 represent [DETR]
%   : MTL - 확장 가능 이유 (unified arch potential) - instance-wise shared representation
%   : query 가 어떤 정보를 포함하는가? 질문 
% 2) 현재 발전 방향 (Detection 위주 - query 에 담는 정보)
%   : DAB-DETR : Detection 위주, 
%      anchor 정보만 포함하였었는데, 이것은 MTL 하기에는 ~ 부족한 점이 있다. 
% 3) MTL 확장의 문제점
%   : 
% 4) new object-centric query design
%   : (핵심 아이디어) explicitly embed box/keypoints into query
%   : prediction head 에도 feed (왜? query 에 high-level 정보가)
%   content query lacks postional/structral information
%      기존 prediction head 에는 content query 만 feed 됐었는데, son's query 에도 중요한 정보가 담겨 있으니 feed 
%   : 이렇게 하면 deformable attention 잘 algin 된다. 
%   we divide query into two 
%   이것은 ~와 포함하는 좋은 design
% 4) More complicated tasks(정의- seg, pose) more than box information 를 다루기 위해 우리가 제안한 방법
% 5) 결론적으로 efficient and accurate}
% Query 관점
% 1) 

% 2) Explicit shape representation 
% 2) Shape == keypoints?}

%% Transformer, object-centric learning
%\park{vit 이야기 없이 detection 이야기 바로 들어가도 되지 않을까?}

% \sol{Detection, Segmentation, Pose를 한 모델에서 해야하는 이유로 시작하면 어떨까요? 세가지를 빠르게 해야하는 이유 등등...
% Top down이 느려서 Bottom up 방식이 나오고 있다.
% Object centric learning을 쓰면 Top down도 빠르게 할 수 있다.
% }

% \son{multi-task 관점에서 시작하면: multi-task network가 중요하고 많이 연구되고 있다. 그 이유는 여러 태스크를 cost-effective 하게 수행할 수 있고 이러한 요구가 있는 상황이 많이 있기 때문 (예시 들기). Pose estimation, segmentation, detection 등의 Instance-wise tasks들의 multi-task learning이 기존에는 어려웠다. (있더라도 task별 overhead가 컸다.) 이는 task마다 다른 pre/post processing을 요구하기 때문이다. Object-centric learning은 이상적으로 효율적으로 이러한 tasks들을 multi-tasking 할 수 있는 구조다. }

% \son{transformer부터 시작의 경우: (이 방향은 아닌듯)
% Transformer가 비전 태스크에서 많이 사용되고 있음. Image feature 뽑는 backbone (ViT, Swin)으로 사용되어 많은 성능 improvement. 최근 detection task를 위주로 object-centric learning이 연구되고 있음. }

% \change{현재 8개 문단}
% \change{human에 집중해서 쓰는거 고려}
%\il{Try to say: Tranditional Multi-task learning vs Object-centric MTL, benefits of object-centric MTL}
%\il{Try to say: difficulties in object-centric MTL and the reason -> how we approach (focusing on query) Interpretation of queries }
%\il{segmentation and pose estimation}

% \son{좀더 표현들을 다듬어야 함}
Multi-task learning is highly demanded in various computer vision fields to reduce redundant computations of multiple tasks. However, cost-efficient multi-tasking of various instance-level vision tasks is not straightforward because they have different task-specific architectures, difficult to be efficiently combined. 
% In this paper, we present a cost-efficient multi-task architecture based on object-centric learning.
% object-centric learning의 개념
Recently, meanwhile, the concept of object-centric learning is presented by \cite{Locatello01,carion2020detr}, which each query in a Transformer layer to map the image feature of a corresponding object instance without pre/post-processing such as region proposal and non-maximal suppression.
It means that downstream tasks can perform in a unified architecture by attaching simple task-specific heads to the object-centric representations.
% and it greatly reduces the computational cost for multi-tasking by exploiting the shared representation.
Despite this potential, multi-tasking based on object-centric learning has been rarely studied.
In this paper, we explore a cost-efficient unified network based on object-centric learning for performing multiple tasks together.
% 학습된 representation에 head를 붙이면 특정 task를 수행가능 하기 때문에, 여러 task를 최대한 computation을 공유하면서 unified architecture로 구성할 수 있는 가능성을 가지고 있음. 그러나 아직 제대로 된 multi-tasking 연구가 되고 있지 않음. Object-centric multi-task learning을 위해 기존 object-centric learning의 분석이 필요.
% Object-centric learning is the concept of 

%% previous query design (content part, positional part)
% \son{좀 더 기존 object-centric query의 발전 방향을 자연스럽고 흥미롭게 서술해야 함}
Na\"ive multi-tasking in object-centric learning would also face performance drops in the tasks. The reason is that an object-centric shared representation consists of mixed information for multiple tasks that can hinder each other of the tasks.
To avoid this problem, we focus on improving an object query design for effective representation learning for multiple tasks.
% Before delving into our proposed design, we first analyze previous an object-centric query design. 
% In query-key cross-attention, a query is considered as two parts; decoder embedding (content part) and learnable query (positional part), according to \cite{liu2022dab}. While early object-centric learning \cite{carion2020detr} adopt the conventional design intactly, 
% In object-centric learning~\cite{carion2020detr,zhu2021deform,liu2022dab,wang2022anchor,cheng2021maskformer,cheng2022mask2former}, 
As analyzed in \cite{liu2022dab}, an object query is structurally interpreted as two parts; decoder embedding (content part) and learnable query (positional part).
In a traditional query-key cross-attention mechanism, the learnable query is considered as an embedding referring to a region which the query focuses on, and is trained to be matched with the positional embedding of target (key) features.
% Learnable query is used to consider the position of a query in computing cross-attention between keys queries, similar to positional embedding of features (key). 
In DETR~\cite{carion2020detr}, the learnable query is the form of a general vector, and the architecture of learnable query barely considers the process of positional embedding of image features. Consequently the model shows a slow convergence speed in training.

To resolve this problem, in the following works~\cite{zhu2021deform,liu2022dab,wang2022anchor}, the query design has improved to explicitly represent positional information of object instances. 
In deformable DETR~\cite{zhu2021deform}, the learnable vector is directly used to predict the reference point coordinates for deformable attentions. In DAB-DETR~\cite{liu2022dab} and Anchor DETR~\cite{wang2022anchor}, they present a learnable anchor representing an object's position and scale, instead of an arbitrary vector.
These query designs make the training convergence much faster by facilitating an attention process. Moreover, as the query explicitly represents bounding box information, these naturally improve the final performance of their object detection models.
% In bbox는 object detection의 output이므로 이러한 query 학습을 통해 자연스럽게 object detection이 수행되고, 성능도 향상됨. (query를 more explicitly
% \son{We notice that, in Deformable DETR, the learnable query does not need to be correlated with positional embedding of a key, by avoiding key-query similarity measure.}
% \son{We notice that, in DAB-DETR, query can learn explicit attributes }

%디텍션 위주로 발전 
%Mask2Former에서는 DETR 구조가 그대로 사용됨 - 언급 필요할지?

%%%--------------------------------------------------------------------------------
\begin{figure*}[ht]
\begin{center}
\includegraphics [width=1.0\linewidth] {figure/method/query_comparison}
\end{center}
\vspace{-12pt}
  \caption{Query design comparison of DETR, Deformable DETR, DAB-DETR and ours.
  For clarity, we visualize a cross-attention function in Transformer decoders mainly and highlight our main differences in green color.
  \son{DAB-DETR논문 처럼 여기서 기술적 변화 및 차이를 잘 설명}
  DETR use ..., 
  Deformable DETR estimate ...
  DAB DETR ...
  However, 
  Regarding the query usages, distinct from all the other methods, our learnable anchor keypoints are fed in downstream task heads directly.
  In addition, (deformable attention 측면)
}
\label{fig:query}
% \vspace{-12pt}
\end{figure*}
%%%--------------------------------------------------------------------------------

%% disadvantage of the previous design for multi-task learning: 1) query가 여러가지 정보를 포함해야함, 2) shape 정보 포함이 애매함, 3) positional part가 downstream task에서 explicit하게 사용되지 않음 
% \son{query가 여러 multi-task 정보를 implicit하게 한번에 학습하는 것은 비효율적이라는 것을 좀 더 직관적으로 표현해야할 것 같음, 지금은 너무 길고 중복적인 내용으로 표현한듯}
However, such design would not be fully suitable to be used for multi-tasking including heterogeneous tasks such as object segmentation and pose estimation.
Such tasks require more complicated information than positional information.
In the end, decoder embedding (content part) should learn all the information for multiple tasks.
% \son{multi-tasking에서 보통 성능이 떨어지는 이유는 shared representation에 각 task 측면에서 성능을 떨어뜨릴 수 있는 요소가 포함되기 때문}
% Many previous works adopt learnable anchor boxes to explicitly represent the positional information of objects for mainly improving a object detection task. However, this form may not provide sufficient information for more complicated tasks, which need to predict more than positional information such as the structure of objects. In the end, other various information including structural information should be implicitly learned in decoder embedding. 
Implicit learning of object structures and other information together would be ineffective, as inferred in the previous object detection works~\cite{liu2022dab,wang2022anchor} that show explicit learning of positional information improve the performance of their tasks. From this perspective, we can expect that explicit representation of object structures as well would lead to performance improvements in other tasks.

% keypoint 정보를 활용해볼까?
However, a compact embedding for an object structure is not straightforward. One na\"{i}ve choice may be to use a mask, but it requires a huge dimension. For example, the object of middle size is composed of over about thousand pixels ($\geq 32\times32$ pixels), but the dimension of the object query is typically $256$ to $512$. On the other hand, sparse keypoints can provide enough semantic and structural information.
%For example,  예를 들어 COCO의 중간 크기 물체만 하더라도 1,000개 이상의 픽셀로 이루어짐. 반면 object query dimension은 보통 256-512. Keypoint를 생각해보면 sparse한 매우 작은 개수의 포인트로 물체의 semantic and structural information을 충분히 제공


%% our solution
Based on the motivation, in this paper, we present a new query design to compactly represent the structural information of objects. To this end, our learnable query carries the coordinates of keypoints for an object along with its bounding box, which is an efficient way to represent the structure of the object. We segregate and represent explicitly the information according to the tasks so that each down-stream head can be trained with ease by utilizing the well-defined high-level information.
% \son{disentangle이라는 표현은 약간 안 맞지만 어쨋든 여러 정보를 explicitly disentangle 시켜서 배움으로써 각 task들이 잘 학습되도록 facilitate, Also, 잘 학습된 high-level information을 활용하는 방법도 제안. }

In previous works, the information of learnable queries is usually used for only computing attentions, and has been barely used in downstream tasks explicitly. It means that the processed query can be regarded as the result itself, or it can be a summarized information of various tasks.
%\son{query 자체가 task의 결과라고 할수도 있고, 여러 task의 결과 정보를 종합하여 사용한다는 의미를 가질수도 있음}
Distinguished from previous methods, we explicitly feed the learnable query into the task heads to exploit the pre-computed high-level information. We observe that this approach improves overall multi-tasking performance. 

%% deformable attention과 align
Furthermore, our learnable anchor keypoints can be utilized for computing attention.
Someone thinks it is strange to include keypoint information in the positional part of a query from the traditional perspective point of view because there has not been no keypoint encoding as tranditional positional encoding does. We solved this problem by using deformable cross-attention. The deforamable attention predicts the sample locations instead of learning direct key-query similarity, so it is better for the query to have more information. 
% \son{추가 내용: positional query가 keypoint를 담는게 전통적인 attention 구조에서는 이상할 수 있음 (query-key(feature) similarity를 구해야 하는데 key는 keypoint를 encoding하지 않기 때문에). 우리는 따라서 cross-attention 방법으로 deformable attention을 사용함으로써 이 문제를 자연스럽게 해결. Deformable attention은 direct key-query similarity를 배우는 것이 아니라 query로부터 sampling locations을 predict하는 구조이기 때문에 qeury가 정보를 많이 담을 수록 더 좋을 수 있음}
Besides, we present a simple but effective way to directly use the learnable anchor keypoints for computing attentions; that is keypoints are good sampling locations for deformable attentions. It also reduces redundant computations for predicting the sampling locations.

Finally, we present a unified network architecture performing heterogeneous human instance-level vision tasks with minimal task overheads.
In the experiment, as our keypoints are trained in a supervised manner, we focus on handling a human class of which labels for all tasks are available.
Our multi-task model achieves comparable accuracy to state-of-the-art task-specific models with smaller computational costs in three tasks; human object detection, pose estimation, and segmentation.
 

To summarize, our contributions include:
\begin{itemize}
    \item A new object-centric query design to effectively represent the structural information of instances,
    % structual (pose) + positional (box)
    \item Explicit utilization of high-level positional and structural information learned in the proposed query for downstream tasks,
    \item Direct utilization of the proposed query for the effective computation of deformable attention,
    \item Demonstration of a cost-efficient unified architecture for multiple human instance-level recognition tasks.
\end{itemize}




